Bridging the Gap Between $f$-GANs and Wasserstein GANs

Generative adversarial networks (GANs) have enjoyed much success in learning high-dimensional distributions. Learning objectives approximately minimize an $f$-divergence ($f$-GANs) or an integral probability metric (Wasserstein GANs) between the model and the data distribution using a discriminator. Wasserstein GANs enjoy superior empirical performance, but in $f$-GANs the discriminator can be interpreted as a density ratio estimator which is necessary in some GAN applications. In this paper, we bridge the gap between $f$-GANs and Wasserstein GANs (WGANs). First, we list two constraints over variational $f$-divergence estimation objectives that preserves the optimal solution. Next, we minimize over a Lagrangian relaxation of the constrained objective, and show that it generalizes critic objectives of both $f$-GAN and WGAN. Based on this generalization, we propose a novel practical objective, named KL-Wasserstein GAN (KL-WGAN). We demonstrate empirical success of KL-WGAN on synthetic datasets and real-world image generation benchmarks, and achieve state-of-the-art FID scores on CIFAR10 image generation.

==> proofs/restrict_fr.tex <==
\begin{proof}
Let us consider $h(u, \vx) := f'(r(\vx)) \cdot u - f(u)$, where $f^{*}(f'(r(\vx))) = \sup_{u \in R} h(u, \vx)$. We have $\partial h / \partial u = f'(r(\vx)) - f'(u)$, since $f$ is convex, $f'$ is non-decreasing, so $\partial h / \partial u$ is zero when $u = r(\vx)$, non-negative when $u < r(\vx)$ and non-positive when $u > r(\vx)$. Therefore, $f^{*}(f'(r(\vx))) = f'(r(\vx)) \cdot r(\vx) - f(r(\vx))$ for all $\vx \in \gX$, and from Lemma~\ref{thm:nwj} we have:
\begin{align}
    D_{f}(P \Vert Q) & = \sup_{T \in L^\infty(Q)} \bb{E}_{P}[T] - \bb{E}_{Q}[f^{*}(T)] \\
    & = \sup_{r \in L^\infty_{\geq 0}(Q)} \bb{E}_{P}[f'(r)] - \bb{E}_{Q}[f^{*}(f'(r))] \label{eq:proof-restrictfr} \\
    & = \sup_{r \in L^\infty_{\geq 0}(Q)} \bb{E}_{P}[f'(r)] - \bb{E}_{Q}[r \cdot f'(r) - f(r)]. \nonumber
\end{align}
where the second equality holds because the optimal $T = f'(\diff P / \diff Q)$ (from Lemma~\ref{thm:nwj}) and $\diff P / \diff Q \in L^{\infty}_{\geq 0}(Q)$ (from the fact that $P \ll Q$, $\forall \vx \in \gX, \vx \in \mathrm{supp}(P) \Rightarrow \vx \in \mathrm{supp}(Q)$, so $\diff P(\vx) / \diff Q(\vx)$ is bounded) so the supremum in \eqref{eq:proof-restrictfr} can be achieved.
\end{proof}

==> statements/dv.tex <==
\begin{corollary}%
$\forall P, Q \in \gP(\gX)$ such that $P \ll Q$,
\begin{align}
    D_{\mathrm{KL}}(P \Vert Q) = \sup_{T\in L^\infty(Q)} \bb{E}_{P}[T] - \log \bb{E}_{Q}[e^T].
    \label{eq:dv}
\end{align}
\end{corollary}

\begin{proof}
$\forall T \in L^\infty(Q)$, we consider $r(T) = e^T / \E_{Q}[e^T]$, where %
$r(T) \in \Delta(Q)$ by definition. If $T = \log (\diff P / \diff Q)$, we have $r(T) = \diff P / \diff Q$. From Proposition~\ref{thm:f-delta-q}:
\begin{align}
    D_{\mathrm{KL}}(P \Vert Q) & =  \sup_{r \in \Delta(Q)} \bb{E}_{P}[\log r + 1] - \bb{E}_{Q}[r] \\
    & = \sup_{T\in L^\infty(Q)} \bb{E}_{P}[T] - \log \bb{E}_{Q}[e^T]
\end{align}
which completes the proof.
\end{proof}

==> statements/f_delta_q.tex <==
\begin{restatable}{proposition}{fdeltaq}
\label{thm:f-delta-q}
$\forall P, Q \in \gP(\gX)$ such that $P \ll Q$,
\begin{align}
    D_{f}(P \Vert Q) &= \sup_{r \in \Delta(Q)} \bb{E}_{P}[f'(r)] - \bb{E}_{Q}[r \cdot f'(r) - f(r)]
    \nonumber \\ %
    &= \sup_{r \in S_{\gF_R}(P, Q)} \bb{E}_{Q}[f(r)],
    \nonumber
\end{align}
and the supremum is achieved when $r = \diff P / \diff Q$.
\end{restatable}

==> statements/f_sfpq.tex <==
\begin{restatable}{proposition}{fsfpq}
\label{thm:f-sfpq}
$\forall P, Q \in \gP(\gX)$ such that $P \ll Q$,
\begin{align}
    D_{f}(P \Vert Q) = \sup_{r \in S_{\gF_R}(P, Q)} \bb{E}_{Q}[f(r)],
    \nonumber %
\end{align}
and the supremum is achieved when $r = \diff P / \diff Q$.
\end{restatable}

==> statements/renyi.tex <==
\begin{restatable}{theorem}{renyi}
\label{thm:renyi}
$\forall P, Q \in \gP(\gX)$ such that $P \ll Q$, and for all $\alpha > 1$, we have
\begin{align}
    &  D_{\alpha}(P \Vert Q) = \sup_{T \in L^\infty(Q)}  \frac{\alpha \log \bb{E}_P[T^{\alpha-1}]}{\alpha - 1}  - \log \bb{E}_{Q}[T^\alpha] \nonumber
\end{align}
where the optimal $r = \diff P / \diff Q$, and
\begin{align}
     D_{\alpha}(P \Vert Q) = \frac{1}{(\alpha-1)} \log \left( \bb{E}_Q\left[\left(\frac{\diff P}{\diff Q}\right)^\alpha - 1\right] \right)
\end{align}
is the R{\'e}nyi $\alpha$-divergence.
\end{restatable}



==> statements/restrict_fr.tex <==
\begin{restatable}{proposition}{restrictfr}
\label{thm:restrictfr}
$\forall P, Q \in \gP(\gX)$ such that $P \ll Q$,
\begin{align}
  \hspace*{-0.1in}  D_{f}(P \Vert Q) = \sup_{r \in L^\infty_{\geq 0}(Q)} \E_{Q}[f(r)] + \bb{E}_{P}[f'(r)] - \bb{E}_{Q}[r \cdot f'(r)]
    \nonumber %
\end{align}
and the supremum is achieved when $r = \diff P / \diff Q$.
\end{restatable}
